On Balancing Bias and Variance in Unsupervised Multi-Source-Free Domain Adaptation

Due to privacy, storage, and other constraints, there is a growing need for unsupervised domain adaptation techniques in machine learning that do not require access to the data used to train a collection of source models. Existing methods for multi-source-free domain adaptation (MSFDA) typically train a target model using pseudo-labeled data produced by the source models, which focus on improving the pseudo-labeling techniques or proposing new training objectives. Instead, we aim to analyze the fundamental limits of MSFDA. In particular, we develop an information-theoretic bound on the generalization error of the resulting target model, which illustrates an inherent bias-variance trade-off. We then provide insights on how to balance this trade-off from three perspectives, including domain aggregation, selective pseudo-labeling, and joint feature alignment, which leads to the design of novel algorithms. Experiments on multiple datasets validate our theoretical analysis and demonstrate the state-of-art performance of the proposed algorithm, especially on some of the most challenging datasets, including Office-Home and DomainNet.

==> Sections/rebuttal.tex <==
\section{Rebuttal}

\subsection{Response to Review-F5Ns:}

\paragraph{(1) Regarding the claim of "balancing bias and variance."}
Our theoretical analysis mainly reveals that the generalization error of the MSFDA problem can be decomposed into bias and variance terms. Furthermore, selective pseudo-labeling can balance this trade-off, as more labeled samples decrease the variance but may increase the bias. 
However, finding the exact sweet spot in the trade-off is non-trivial as unknown terms are in the upper bound. Therefore, a more practical solution is to jointly optimize all terms in the generalization error upper bound, which approximately achieves a good balance. Characterizing the exact balance is worth pursuing in future work but might be beyond the scope of the current contribution. We will clarify this point in the revision.


% Our theoretical analysis mainly reveals a trade-off between bias and variance, and balancing such trade-offs is beneficial for the MSFDA problem. However, even in theory, finding the exact sweet-spot in the trade-off is non-trivial as there is an unknown constant term in the upper bound. Therefore, in practice, the more realistic solution is to jointly optimize both the bias and variance, aiming to optimize the generalization error upper bound. To this end, we agree with the reviewer that using "balancing" might be ambiguous, we might consider rephrase the corresponding claim in this work.
% (\textcolor{red}{TODO Yuheng})




\paragraph{(2) Compare with SOTA semi-supervised methods.}
We agree with the reviewer that the "selective oracle" concept might be relevant to semi-supervised learning. However, to our knowledge, there is no existing work trying to address the source-free domain adaptation problem with semi-supervised learning. The most relevant setting is semi-supervised domain adaptation methods (SSDA) [1, 2]. However, it is not reasonable to directly compare our proposed method with SSDA methods due to the distinct problem settings. SSDA assumes that the source data and some labels of target domain data are available. For our MSFDA problem, only the pretrained models from the source domains are available, and none of the data from the target domain is labeled, which is different from SSDA. To this end, MSFDA is a  more difficult problem, but some ideas from SSDA can inspire us to design better selection rules.

[1] Saito, K. Semi-supervised domain adaptation via minimax entropy. (CVPR 2019)

[2] Singh, A. CLDA: Contrastive learning for semi-supervised domain adaptation (NeurIPS 2021)


\paragraph{(3) Extend ablation study.}
% Thanks for the reviewer's suggestion, 

We address the reviewer's concerns about the ablation study as follows: (1) The ablation study of using uniform domain weights is provided in the original submission, i.e., "w/o Domain Weights" in Table 5. We will make this baseline comparison more evident in the revision. (2) As described in section 5.2 and Algorithm 1, the confidence threshold $\alpha_N$ is set to be $N$-th largest confidence score, and we linearly increase $N$ during each epoch until $N=n$. The default value of initial $\alpha$ is set to be the averaged confidence score of all data. In practice, we find such initialization works well for all the datasets. (3) As the reviewer suggests, we conduct an additional ablation study of the total epochs. The results are shown in the following table. It can be observed that training more epochs will achieve better performance. Intuitively, a small epoch means that more samples will be added to $\mathcal{D}_l$ in each iteration, which might introduce more bias as the pseudo-labels are unreliable at the early stage of training.
\begin{table}[h]
  \begin{center}
  \tiny
  \captionsetup{font=small}
  \caption{\textbf{Ablation Study (Total Epochs) on Office-Home}}
  \vspace{-1em}
  \begin{tabular}{lllllll}
    \\
    \toprule
     \textbf{Method} & \makecell{\textbf{C,R,P} \\ $\rightarrow$ \textbf{A}} & \makecell{\textbf{A,R,P} \\ $\rightarrow$ \textbf{C}} & \makecell{\textbf{A,C,P} \\ $\rightarrow$ \textbf{R}} &\makecell{\textbf{A,C,R}\\ $\rightarrow$ \textbf{P}} &\textbf{Avg}\\ 
    \hline
    epoch=5 & 74.6 & 61.4 & 84.1 & 84.4 & 76.1\\
    epoch=10 & 75.5 & 61.3 & 84.0 & 85.2 & 76.5\\
    epoch=20 & 76.1 & 63.2 & 84.8 &85.3 & 77.3\\
    \toprule
  \end{tabular}
  \label{table: Ablation}
  \end{center}
  \vspace{-2em}
\end{table}
\paragraph{(4) Regarding datasets other than standardized domain adaptation datasets.}
We focus on the standard domain adaptation benchmark datasets, as it allows for a more accurate comparison of our proposed method with existing MSFDA approaches. In our experiment, we already used a large-scale dataset DomainNet, which contains about half-million images and can be viewed as the counterpart of traditional large-scale image classification benchmark (e.g., ImageNet) for the domain adaptation problem. Therefore, we believe that the proposed approach, which achieves strong performance on DomainNet, can also generalize well on other large-scale datasets and even real-world datasets.



\subsection{Response to Review-mUiB:}

\paragraph{(1) Regarding the analysis of the limitation of SOTA methods.}
In the revision, we will add the following discussion in the related work section. The algorithm design of most existing MSFDA works tends to be ad-hoc and often lacks theoretical justification. Our work aims to design good MSFDA algorithms by analyzing the MSFDA problem using information-theoretical tools. Although [1] also includes some theoretical analysis, their results require specific assumptions, such as the meta-assumption of the data distribution. Our theoretical result is more general and does not require additional assumptions of the data distribution or models. 


[1] Dong, J Et al. Confident Anchor-Induced Multi-Source Free Domain Adaptation. (NeurIPS2021)

\paragraph{(2) Regarding experiment details.}
We have provided the experimental details, including the learning rate, optimizer, batch size, hyper-parameter of each loss, and other implementation details in Appendix B.3. 
We would be happy to provide any missing experiment details if the reviewer has additional suggestions.

\paragraph{(3) Experimental validation.}
We have provided several aspects of experimental validation suggested by the reviewer in Appendix B.3 of the original submission, including the impact of domain numbers, diversity, and domain shifts on performance. We will make these additional results more visible in the revised paper. 

For other aspects the reviewer suggested, such as the number of classes or the class in-balanced situation, it is difficult to investigate them using existing benchmark datasets comprehensively. We would greatly appreciate any suggestions from the reviewer regarding multi-source DA literature that has conducted a similar experimental validation on these aspects.

Regarding the effect of the number of source samples, we note that the number of source data samples cannot be controlled in a source-free setting. As for the effect of the number of target data samples, an increase in target data samples will not influence the bias term but will reduce the variance term. Consequently, it is reasonable to expect a performance improvement with more target data samples.

% It would be helpful for us to further improve our experiment if the reviewer could suggest a multi-source DA literature that conducts a similar experimental validation as the reviewer suggested.


\paragraph{(4) Regarding time and memory complexity.}
We compare the training time of our method and other SOA methods on the Office-Home dataset in the following table. Our method requires relatively more training time, but it is still in a reasonable range, as each task can be completed within 6 hours. We further compare the number of model parameters as follows: Ours (72,198,858), DECISION (72,149,577), and CaiDA (72,149,578). Our method requires comparable memory storage as other methods.

\begin{table}[h]
  \begin{center}
  \tiny
  \captionsetup{font=small}
  \caption{\textbf{Training Time (Runtime in seconds)}}
  %\caption{\textbf{Ablation Study Results on Office-Home:} w/o alignment and w/o denoise denote the performance without the domain alignment loss and without pseudo-label denoise method, respectively.}
  \vspace{-1em}
  \begin{tabular}{lllll}
    \\
    \toprule
   \textbf{Method} & \makecell{\textbf{C,R,P} \\ $\rightarrow$ \textbf{A}} & \makecell{\textbf{A,R,P} \\ $\rightarrow$ \textbf{C}} & \makecell{\textbf{A,C,P} \\ $\rightarrow$ \textbf{R}} &\makecell{\textbf{A,C,R}\\ $\rightarrow$ \textbf{P}} \\ 
    \hline
    DECISION & 2634.2 s & 2893.4 s & 10352.4 s & 2636.1 s \\
    CAiDA & 1869.7 s & 2153.1 s & 6673.4 s & 2259.6 s \\
    Ours  & 5056.1 s & 5127.9 s & 20004.1 s & 5583.4 s \\
    \toprule
  \end{tabular}
  \label{table: Ablation}
  \end{center}
  \vspace{-2em}
\end{table}

\paragraph{(5) "Tables should show lower-bound and also upper-bound results."}
We already included both the lower-bound and upper-bound results for all the datasets. The baseline "Source-ens" denotes the lower-bound results without any domain adaptation. The "selective oracle" results correspond to the upper-bound results. We will clarify that these two baselines can be interpreted as lower and upper bounds on the MSFDA performance in the revision. 

\paragraph{(6) Regarding how to select the hyper-parameter N .}
We do not require a validation set to tune $\alpha_N$. As described in section 5.2 and Algorithm 1, the confidence threshold $\alpha_N$ is set to be $N$-th largest confidence score, and we linearly increase $N$ for each epoch. The default value of initial $\alpha$ is set to be the averaged confidence score of all data. In practice, we find such initialization works well for all the datasets. While a better selection rule, such as an adaptive update of $\alpha_N$, may exist, we consider finding a more effective surrogate selection rule an intriguing direction for future research, as highlighted in our conclusion section.


% There might exist a better selection rule, such as an adaptive update of $\alpha_N$. As we mentioned in the conclusion section, identifying a more effective surrogate selection rule can be an interesting future work.

\subsection{Response to Review-emvW:}

\paragraph{(1) Novelty of learning domain weights.}
We agree with the reviewer that the general idea of learning domain weights is not new, as the existing SOTA works [1, 2] also consider various ways to learn domain weights. However, finding good domain weights remains a challenging problem worth further investigation. Our work provides theoretical justification for learning domain weights. Specifically, we show that learning better domain weights can effectively reduce the label mismatch bias. 

% We leave proposing other more advanced aggregation approaches as future work.

[1] Ahmed, S. M Et al. Unsupervised multi-source domain adaptation without access to source data. (CVPR2021)

[2] Dong, J Et al. Confident Anchor-Induced Multi-Source Free Domain Adaptation. (NeurIPS2021)

\paragraph{(2) Better solution for changing confidence parameter N.}

We agree with the reviewer that designing a more advanced query strategy will benefit the performance of the MSFDA problem, as it works as a surrogate of the "selective oracle" to close the gap between theory and practice. We try to investigate this by changing the linear update rule to an adaptive one. Specifically, we use a step decay method that decays the confidence threshold for each epoch, which is motivated by the intuition that it might be better to query more data later as the pseudo label will be more reliable than the early stage training. However, as shown in the following table, the adaptive update rule does not show apparent benefits compared to the linear update. To this end, as highlighted in our conclusion section, finding a more effective surrogate selection rule is an intriguing direction for future research.
\begin{table}[h]
  \begin{center}
  \tiny
  \captionsetup{font=small}
  \caption{\textbf{Ablation Study (query strategy) on Office-Home}}
  \vspace{-1em}
  \begin{tabular}{lllllll}
    \\
    \toprule
     \textbf{Method} & \makecell{\textbf{C,R,P} \\ $\rightarrow$ \textbf{A}} & \makecell{\textbf{A,R,P} \\ $\rightarrow$ \textbf{C}} & \makecell{\textbf{A,C,P} \\ $\rightarrow$ \textbf{R}} &\makecell{\textbf{A,C,R}\\ $\rightarrow$ \textbf{P}} &\textbf{Avg}\\ 
    \hline
    step-decay & 75.8 & 62.3 & 84.4 & 85.5 & 77.0\\
    Ours & 76.1 & 63.2 & 84.8 &85.3 & 77.3\\
    \toprule
  \end{tabular}
  \label{table: Ablation}
  \end{center}
  \vspace{-2em}
\end{table}

\paragraph{(3) Regarding the readability of the paper and the framework diagram.}
We thank the reviewer's suggestion to help us further improve the readability of our work. We will revise the framework diagram in the revised version.


\paragraph{(4) Regarding the effects of data augmentation on bias-variance trade-off.}
We agree with the reviewer that the data augmentation might affect the label mismatch bias. In order to investigate this issue, we conduct an ablation study of data augmentation by evaluating the performance of our proposed method without using data augmentation. The results are shown in the following table. It can be observed that the performance degrades without data augmentation, which empirically demonstrates that data augmentation can reduce the variance term while the effects on the label mismatch bias are minor.
\begin{table}[h]
  \begin{center}
  \tiny
  \captionsetup{font=small}
  \caption{\textbf{Ablation Study (Data Argumentation) on Office-Home}}
  \vspace{-1em}
  \begin{tabular}{lllllll}
    \\
    \toprule
     \textbf{Method} & \makecell{\textbf{C,R,P} \\ $\rightarrow$ \textbf{A}} & \makecell{\textbf{A,R,P} \\ $\rightarrow$ \textbf{C}} & \makecell{\textbf{A,C,P} \\ $\rightarrow$ \textbf{R}} &\makecell{\textbf{A,C,R}\\ $\rightarrow$ \textbf{P}} &\textbf{Avg}\\ 
    \hline
    w/o augmentation & 75.1 & 61.6 & 84.1 & 84.5 & 76.3\\
    Ours & 76.1 & 63.2 & 84.8 &85.3 & 77.3\\
    \toprule
  \end{tabular}
  \label{table: Ablation}
  \end{center}
  \vspace{-2em}
\end{table}

\paragraph{(5) Regarding algorithm efficiency.}
We compare the training time of our method and other SOA methods on the Office-Home dataset in the following table. Our method requires relatively more training time, but it is still in a reasonable range, as each task can be completed within 6 hours. We further compare the number of model parameters as follows: Ours (72,198,858), DECISION (72,149,577), and CaiDA (72,149,578). Our method requires comparable memory storage as other methods.

\begin{table}[h]
  \begin{center}
  \tiny
  \captionsetup{font=small}
  \caption{\textbf{Training Time (Runtime in seconds)}}
  %\caption{\textbf{Ablation Study Results on Office-Home:} w/o alignment and w/o denoise denote the performance without the domain alignment loss and without pseudo-label denoise method, respectively.}
  \vspace{-1em}
  \begin{tabular}{lllll}
    \\
    \toprule
   \textbf{Method} & \makecell{\textbf{C,R,P} \\ $\rightarrow$ \textbf{A}} & \makecell{\textbf{A,R,P} \\ $\rightarrow$ \textbf{C}} & \makecell{\textbf{A,C,P} \\ $\rightarrow$ \textbf{R}} &\makecell{\textbf{A,C,R}\\ $\rightarrow$ \textbf{P}} \\ 
    \hline
    DECISION & 2634.2 s & 2893.4 s & 10352.4 s & 2636.1 s \\
    CAiDA & 1869.7 s & 2153.1 s & 6673.4 s & 2259.6 s \\
    Ours  & 5056.1 s & 5127.9 s & 20004.1 s & 5583.4 s \\
    \toprule
  \end{tabular}
  \label{table: Ablation}
  \end{center}
  \vspace{-2em}
\end{table}



\subsection{Response to Reviewer-LeEs:}
\paragraph{(1) Regarding the notations and line 159.}
While our theoretical analysis may be dense and involve numerous notations, we have presented our theoretical derivation clearly and have well-defined notations. We will strive to make our notation system more accessible in the revision.

In the MSFDA problem, the source domain data is not available, but multiple pretrained source domain models are given, and our goal is to adapt these pretrained source models to the target domain. In our notation system, we use superscript $s_j$ to denote something obtained from the $j$-th source domain model. More specifically, we use $\bm{f}^{s_j}$, and $\bm{g}^{s_j}$ to denote \emph{feature extractor} and \emph{classifier} of $j$-th source domain pretrained model, respectively. In line 159, we use $\bm{\phi}_i^{s_j}$ to denote the \textbf{feature of target data} $\bm{x}_i^t$ extracted using $j$-th \textbf{source domain} \emph{feature extractor}. 

In addition, we use $P^{s_j}_{Y|\Phi_j=\phi_j}$ to denote the label distribution conditioned on feature $\bm{\phi}^{s_j}$, induced by $j$-th \textbf{source domain} \emph{classifier}. We use $P^{\gD_l}_{Y|\Phi_{1:m}}$ to denote the labeling distribution we aim to construct by aggregating information obtained from all the source models. 

We hope the above explanation can resolve any potential misunderstandings, and we would like to provide further clarification if the reviewer has additional questions about the notations.

\paragraph{(2) Clarify the bias.}
The reviewer might have a potential misinterpretation of the notations and terms defined in Theorem 4.1. To avoid any confusion for the general audience, we would like to provide more explanation about the bias and variance under Theorem 4.1 for clarification.

The labeling distribution $P^{\mathcal{D_l}}_{Y|\Phi_{1:m}}$ defines the pseudo labeling distribution on the target domain, constructed from multiple source domain pretrained models. Similarly, the marginal feature distribution $P^{\mathcal{D_l}}_{\Phi_{1:m}}$ defines the joint feature representation of the target domain induced from multiple source domain feature extractors. These two quantities do not depend on source domain data distributions, i.e., $\{P^{s_j}_{XY}\}_{j=1}^m$. Therefore, the label distribution mismatch bias quantifies the discrepancy between the constructed labeling distribution and the target domain ground-truth labeling distribution instead of measuring the discrepancy of label distribution from different domains. Similarly, the feature misalignment bias measures the misalignment of marginal feature distribution of the target domain induced from the source models instead of directly quantifying the distribution shift between target and source domains. 





\paragraph{(3) Other ways to quantify the variance term.}
% (\textcolor{red}{TODO Yuheng})
The variance term depends on both model complexity and the number of labeled samples in $\mathcal{D}_l$. As explained in section 4.2, the model complexity is fixed, while the number of labeled samples is controlled by the algorithm. The selective Oracle (definition 1) and our proposed surrogate selection technique in section 5.2 aim to select more data in $\mathcal{D}_l$ to reduce the variance while balancing the bias terms. Unlike distribution shift and model complexity, which are fixed quantities solely determined by domain data distributions and the model itself, the bias and variance defined in this work are controllable and can be jointly optimized by the algorithm design.


Moreover, as Rademacher complexity and VC dimension are defined only for binary classification, the approach employed in our work, i.e., the Natarajan dimension, which generalizes the VC dimension to the multi-class case, is a more suitable measure of model complexity in this paper.

% The better way to measure model complexity is not crucial for source-free domain adaptation problem and is the not the focus of this work. 

% Rademacher complexity is typically used for binary classification.
% Natarajan dimension is the generalization of VC dimension for multiclass case, while  Rademacher complexity is used for binary classification.

\paragraph{(4) Compare with baseline with more advanced ensemble method such as Bagging or Boosting.}
We have already compared our proposed method with a simple baseline aggregating multiple source models using uniform weights, similar to bagging, denoted as "Source-ens" in the table. In addition, we have compared our method with other SOTA MSFDA approaches [1, 2]. These SOTA approaches are specifically designed to address the MSFDA problem and can achieve better performance than naive approaches like boosting or bagging, while our proposed method still demonstrates the advantages over the SOTA methods. We will clarify the compared baselines in the revision. 






\paragraph{(5) The performance of using equal weights for each model.}
Other MSFDA approaches, including SOTA works [1, 2] that we already compared in our experiments, employ learnable weights to aggregate multiple domains, which can yield better results than uniform weights. Our ablation study further demonstrated that using uniform weights decreases performance compared to learnable weights. Therefore, we believe that it is not necessary for additional comparisons with other MSFDA approaches using uniform weights.


\paragraph{(6) Regarding data augmentation for other methods.}
The data augmentation technique used in this work is motivated by our theoretical analysis, i.e., increasing the training data in $\mathcal{D}_l$ will reduce the variance term. Other methods compared in the experiments do not use data augmentation. However, we have conducted an ablation study to demonstrate the performance of our proposed method without data augmentation. The following table shows that even without data augmentation (denoted as w/o augmentation), our proposed method can still outperform other baselines.



\begin{table}[h]
  \begin{center}
  \tiny
  \captionsetup{font=small}
  \caption{\textbf{Ablation Study (Data Argumentation) on Office-Home}}
  \vspace{-1em}
  \begin{tabular}{lllllll}
    \\
    \toprule
     \textbf{Method} & \makecell{\textbf{C,R,P} \\ $\rightarrow$ \textbf{A}} & \makecell{\textbf{A,R,P} \\ $\rightarrow$ \textbf{C}} & \makecell{\textbf{A,C,P} \\ $\rightarrow$ \textbf{R}} &\makecell{\textbf{A,C,R}\\ $\rightarrow$ \textbf{P}} &\textbf{Avg}\\ 
    \hline
    DECISION[1] & 74.5 & 59.4 & 83.6 & 84.4 & 75.5\\
    CAiDA[2] & 75.2 & 60.5 & 84.2 & 84.7 & 76.2\\
    NRC[3] &70.6 &60.0 &84.6 &83.5 &74.7\\
    w/o augmentation & 75.1 & 61.6 & 84.1 & 84.5 & 76.3\\
    Ours & 76.1 & 63.2 & 84.8 &85.3 & 77.3\\
    \toprule
  \end{tabular}
  \label{table: Ablation}
  \end{center}
  \vspace{-2em}
\end{table}


[1] Ahmed, S. M Et al. Unsupervised multi-source domain adaptation without access to source data. (CVPR2021)

[2] Dong, J Et al. Confident Anchor-Induced Multi-Source Free Domain Adaptation. (NeurIPS2021)

[3] Yang, S Et al. Exploiting the intrinsic neighborhood structure for source-free
domain adaptation. (NeurIPS2021)
